Deep learning of parameterized equations with applications to uncertainty quantification

We propose a numerical method for discovering unknown parameterized dynamical systems by using observational data of the state variables. Our method is built upon and extends the recent work of discovering unknown dynamical systems, in particular those using deep neural network (DNN). We propose a DNN structure, largely based upon the residual network (ResNet), to not only learn the unknown form of the governing equation but also take into account the random effect embedded in the system, which is generated by the random parameters. Once the DNN model is successfully constructed, it is able to produce system prediction over longer term and for arbitrary parameter values. For uncertainty quantification, it allows us to conduct uncertainty analysis by evaluating solution statistics over the parameter space.

==> Setup_091019.tex <==
\section{Problem Setup} \label{sec:setup}
We are interested in studying the following differential equation with stochastic parameters.

\begin{equation}
\label{eq:ode}
\frac{d}{dt}\x(t, \omega)=\f(\x, \aalpha(t, \omega)), \quad \x(0)=\x_0,
\end{equation}
where $\x \in \R^d$ are sate variables with coordinates 
$(x_1, x_2, \ldots, x_d)$ and $\aalpha(\omega)\in \R^l$ are time-dependent random parameters with coordinates $(\alpha_1(t, \omega), \alpha_2(t, \omega),\ldots, \alpha_l(t, \omega))$. 
We further assume that each state variable $x_i(t, \omega)\in [a_i, b_i]$ and each random parameter is contained in $[p_i, q_i]$ for any $t$ and $\omega$. For the random parameters, we assume they are piecewise constant in time and each parameter $\alpha_i(t, \omega)$ can be parameterized by a sequence of random vectors $(\Delta_i, a_i)$, where $\Delta_i\sim U(0, \Delta)$ and $a_i\sim U(0, a)$. If we define 
\begin{equation*}
	t_n=\sum_{i=1}^n \Delta_i
\end{equation*}
then the random parameter $\alpha_i(t,\omega)=a_n$ if $t_n\leq t< t_{n+1}$.
We are interested in quantifying the uncertainty in the solution $\x(T, \Delta_1, a_1, \Delta_2, a_2, \ldots, \Delta_N, a_N)$ for $T>0$.

==> uq.tex <==
\section{Theoretical Properties and Uncertainty Quantification}\label{sec:uq}

